PhD: A ChatGPT-Prompted Visual hallucination Evaluation Dataset

Multimodal Large Language Models (MLLMs) hallucinate, resulting in an emerging topic of visual hallucination evaluation (VHE). This paper contributes a ChatGPT-Prompted visual hallucination evaluation Dataset (PhD) for objective VHE at a large scale. The essence of VHE is to ask an MLLM questions about specific images to assess its susceptibility to hallucination. Depending on what to ask (objects, attributes, sentiment, etc.) and how the questions are asked, we structure PhD along two dimensions, i.e. task and mode. Five visual recognition tasks, ranging from low-level (object / attribute recognition) to middle-level (sentiment / position recognition and counting), are considered. Besides a normal visual QA mode, which we term PhD-base, PhD also asks questions with specious context (PhD-sec) or with incorrect context ({PhD-icc), or with AI-generated counter common sense images (PhD-ccs). We construct PhD by a ChatGPT-assisted semi-automated pipeline, encompassing four pivotal modules: task-specific hallucinatory item (hitem) selection, hitem-embedded question generation, specious / incorrect context generation, and counter-common-sense (CCS) image generation. With over 14k daily images, 750 CCS images and 102k VQA triplets in total, PhD reveals considerable variability in MLLMs' performance across various modes and tasks, offering valuable insights into the nature of hallucination. As such, PhD stands as a potent tool not only for VHE but may also play a significant role in the refinement of MLLMs.

==> AnonymousSubmission/tables/tab-exp-context.tex <==
\begin{table}[ht]
    \centering
    \ra{1.1}
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{@{}lrrrrrrrrr@{}}
        \toprule
        \multirow{2}{*}{\textbf{Model}}& \textbf{wo context} & \multicolumn{4}{c}{\textbf{w implicit context}} & \multicolumn{4}{c}{\textbf{w explicit context}} \\
        \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(l){7-10}
        & PhD-S. & Yes-R. & No-R. & Acc & PhD-S. & Yes-R. & No-R. & Acc & PhD-S. \\
        \midrule
        LLaVA-1.5 &  &  &  &  &  &  &  &  \\
        Qwen-VL &  &  &  &  &  &  &  &  \\
        InstructBLIP &  &  &  &  &  &  &  &  \\
        MiniGPT-v2 &  &  &  &  &  &  &  &  \\
        MPlug-owl2 &  &  &  &  &  &  &  &  \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Comparison of Models with Different Contexts}
\end{table}

==> AnonymousSubmission/tables/tab-statistic-bak.tex <==
\begin{table*}[h]
    \begin{subtable}[b]{0.52\textwidth}
    \fontsize{14pt}{15pt}\selectfont
    \ra{1.2}
        \centering
        \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{@{}lrrrrrrr@{}}
            \toprule
            & \multicolumn{5}{c}{\textbf{Tasks}} & \multicolumn{2}{c}{\textbf{Questions}} \\
            \cmidrule(lr){2-6} \cmidrule(lr){7-8} 
            & \textit{Object} & \textit{Attribute} & \textit{Sentiment} & \textit{Position} & \textit{Counting} & \textit{Yes} & \textit{No} \\
            \hline
            \#TDIUC samples used &6,271 &4,324	&2,095&	2,841 & 3,387 & n.a. & n.a. \\
            \emph{Manual correction rate} &  8.5\% & 7.6\% & 15.3\% & 12.3\% & 16.0\% & n.a. & n.a. \\ [2pt]
            \#unique hitems & 745 & 146 & 65 & 486 & 10 & n.a. & n.a. \\
            \#VQA triplets generated & 11,472 & 7,994 & 3,550 & 4,984 & 5,688 & 16,844 & 16,844 \\
            \#VQA w/ inaccurate context & 11,472 & 7,994 & 3,550 & 4,984 & 5,688 & 16,844 & 16,844 \\
            \#VQA w/ incorrect context & 11,472 & 7,994 & 3,550 & 4,984 & 5,688 & 16,844 & 16,844 \\
            \#VQA w/ CCS images & 172	&367	&39	&110	&62 & 750 & 750 \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        \caption{Data statistics of \texttt{PhD}}
        
    \end{subtable}%
    \hspace{0.2cm}
    \begin{subtable}[b]{0.46\textwidth}
    \fontsize{14pt}{15pt}\selectfont
    \ra{1.35}
        \centering
        \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{@{}lrrrrrr@{}}
            \toprule
            \textbf{Benchmark} & \textbf{Daily images} & \textbf{CCS images} & \textbf{Hitems} & \textbf{Contexts} & \textbf{VQA triplets} & \textbf{Tasks} \\
            \hline
            POPE & 500 & \xmark & 80 & \xmark & 3,000 & Obj. \\
            \hline
            Nope &	unknown &	\xmark &	unknown &	\xmark	&  32,701 &	Obj. \\
            \hline
            CIEM &	4,929 &	\xmark &	unknown &	\xmark & 72,941 &	 Obj. / Attr. / Pos. \\
            \hline
            AMBER & 1,004 & \xmark & 687 & \xmark & 14,216 & \makecell[r]{Obj. / Attr./ Pos./\\ Count.} \\
            \hline
            PhD & 14,648 & 750 & 1,452 & 33,688 & 102,564 & \makecell[r]{Obj / Attr. / Pos./\\ Sent. / Count.} \\
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        % \vspace{18px}
        \caption{Comparison with peer benchmarks}
    \end{subtable}
    \caption{\textbf{Data overview}. \texttt{PhD} is substantially larger, more diverse and thus more challenging than its peers.}
     \label{tab:statistic}
\end{table*}

==> AnonymousSubmission/tables/table-exp-all.tex <==
\begin{table*}[ht]
\fontsize{16pt}{16pt}\selectfont
\ra{1.4}

    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{@{}lrrrrrrrrrrrrrrr@{}}
        \toprule
        \multirow{2}{*}{\textbf{MLLM}} & \multirow{2}{*}{\makecell[r]{\textbf{Visual} \\ \textbf{encoder}}} & \multirow{2}{*}{\makecell[r]{\textbf{LLM} \\ \textbf{kernel}}} & \multicolumn{3}{c}{\textbf{PhD-base}} & \multicolumn{3}{c}{\textbf{PhD-sec}} & \multicolumn{3}{c}{\textbf{PhD-icc}} & \multicolumn{3}{c}{\textbf{PhD-ccs}} &  \multirow{2}{*}{\makecell[c]{\textbf{PhD}\\ \textbf{Index}}} \\
        \cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){10-12} \cmidrule(lr){13-15}
        & & & \makecell[c]{Yes-Recall} & \makecell[c]{No-Recall} & PhD Index & \makecell[c]{Yes-Recall} & \makecell[c]{No-Recall} & PhD Index & \makecell[c]{Yes-Recall} & \makecell[c]{No-Recall} & PhD Index & \makecell[c]{Yes-Recall} & \makecell[c]{No-Recall} & PhD Index &\\
        \midrule

 GPT-4o& --	&	--& 0.83$\pm$ 0.09&	0.86$\pm$ 0.09	&0.84$\pm$ 0.08 &	0.80$\pm$ 0.11 &	0.86$\pm$ 0.11 &	0.83$\pm$ 0.10 &0.70$\pm$ 0.13 &	0.87$\pm$ 0.13 &	0.77$\pm$ 0.12	&0.75$\pm$ 0.09 &	0.84$\pm$ 0.09 &	0.79$\pm$ 0.09	&0.81\\ 

Claude 3.5 Sonnet & --	&	--& 0.75$\pm$ 0.11	& 0.78$\pm$ 0.11& 	0.76$\pm$ 0.10& 
0.72$\pm$ 0.08& 	0.88$\pm$ 0.08& 	0.79$\pm$ 0.09& 
0.67$\pm$ 0.12& 	0.85$\pm$ 0.12& 	0.73$\pm$ 0.15& 
0.66$\pm$ 0.12& 	0.77$\pm$ 0.12& 	0.71$\pm$ 0.08 & 0.75\\

Gemini 1.5 Pro  & --	& -- & 0.81$\pm$ 0.08 & 0.85$\pm$ 0.08 & 0.83$\pm$ 0.10 & 
0.64$\pm$ 0.07 & 0.88$\pm$ 0.07 & 0.73$\pm$ 0.12 & 
0.50$\pm$ 0.12 & 0.74$\pm$ 0.12 & 0.56$\pm$ 0.24 & 
0.55$\pm$ 0.11 & 0.79$\pm$ 0.11 & 0.64$\pm$ 0.05 & 0.69\\

 Qwen-VL (Woodpecker) & -bigG/14	& Qwen-7B & 0.63$\pm$ 0.12 & 0.59$\pm$ 0.12 & 0.59$\pm$ 0.07 & 
0.61$\pm$ 0.20 & 0.54$\pm$ 0.20 & 0.53$\pm$ 0.10 & 
0.58$\pm$ 0.06 & 0.78$\pm$ 0.06 & 0.65$\pm$ 0.09 & 
0.28$\pm$ 0.12 & 0.64$\pm$ 0.08 & 0.39$\pm$ 0.11 & 0.53\\

 LLaVA-1.6-L (Woodpecker)  & -L/14	& Vicuna-13B-1.5  & 0.59$\pm$ 0.30 & 0.46$\pm$ 0.30 & 0.44$\pm$ 0.29 & 
0.41$\pm$ 0.09 & 0.82$\pm$ 0.09 & 0.52$\pm$ 0.14 & 
0.40$\pm$ 0.31 & 0.71$\pm$ 0.31 & 0.44$\pm$ 0.23 & 
0.17$\pm$ 0.09 & 0.80$\pm$ 0.11 & 0.29$\pm$ 0.12 & 0.41\\
 
\hline

LLaVA-OneVision & SoViT-400m/14 &Qwen2-72B &0.84$\pm$ 0.09 & 0.73$\pm$ 0.09 & 0.78$\pm$ 0.07 &  
0.76$\pm$ 0.11 & 0.64$\pm$ 0.11 & 0.69$\pm$ 0.09 &  
0.69$\pm$ 0.13 & 0.59$\pm$ 0.13 & 0.63$\pm$ 0.12 &  
0.69$\pm$ 0.11 & 0.71$\pm$ 0.11 & 0.70$\pm$ 0.07 &  0.70\\

Molmo & -L/14& Qwen2-72B & 0.84$\pm$ 0.13 & 0.65$\pm$ 0.13 & 0.73$\pm$ 0.11 &  
0.62$\pm$ 0.10 & 0.82$\pm$ 0.10 & 0.70$\pm$ 0.11 &  
0.51$\pm$ 0.09 & 0.78$\pm$ 0.09 & 0.60$\pm$ 0.16 &  
0.67$\pm$ 0.07 & 0.84$\pm$ 0.07 & 0.74$\pm$ 0.04 & 0.69 \\

InternVL-1.5& InternViT-6B &InternLM2-20B &0.89$\pm$ 0.13 & 0.66$\pm$ 0.13 & 0.75$\pm$ 0.09 &  
0.55$\pm$ 0.11 & 0.64$\pm$ 0.11 & 0.59$\pm$ 0.15 &  
0.39$\pm$ 0.11 & 0.31$\pm$ 0.11 & 0.30$\pm$ 0.16 &  
0.48$\pm$ 0.10 & 0.80$\pm$ 0.10 & 0.60$\pm$ 0.09 & 0.56\\

Qwen-VL (VCD) &-bigG/14& Qwen-7B & 0.81$\pm$ 0.08 & 0.71$\pm$ 0.08 & 0.76$\pm$ 0.07 &  
0.59$\pm$ 0.16 & 0.50$\pm$ 0.16 & 0.50$\pm$ 0.14 &  
0.52$\pm$ 0.09 & 0.22$\pm$ 0.09 & 0.28$\pm$ 0.12 &  
0.74$\pm$ 0.12 & 0.68$\pm$ 0.12 & 0.71$\pm$ 0.09 & 0.56\\

Cambrian-1& Hybrid &Llama-3-8B& 0.85$\pm$ 0.11 & 0.66$\pm$ 0.11 & 0.74$\pm$ 0.09 &  
0.65$\pm$ 0.09 & 0.44$\pm$ 0.09 & 0.52$\pm$ 0.10 &  
0.55$\pm$ 0.12 & 0.24$\pm$ 0.12 & 0.30$\pm$ 0.14 &  
0.60$\pm$ 0.14 & 0.68$\pm$ 0.14 & 0.63$\pm$ 0.10 & 0.55\\

LLaVA-1.6-L (VCD) &-L/14 &Vicuna-13B-1.5& 0.81$\pm$ 0.08 & 0.59$\pm$ 0.08 & 0.68$\pm$ 0.07 &  
0.63$\pm$ 0.08 & 0.34$\pm$ 0.08 & 0.44$\pm$ 0.09 &  
0.55$\pm$ 0.05 & 0.20$\pm$ 0.05 & 0.29$\pm$ 0.07 &  
0.71$\pm$ 0.10 & 0.58$\pm$ 0.10 & 0.64$\pm$ 0.08 & 0.51\\

LLaVA-1.6-XL& -L/14 &Nous-Hermes-2-Yi-34B &0.78$\pm$ 0.12 & 0.57$\pm$ 0.12 & 0.65$\pm$ 0.09 &  
0.70$\pm$ 0.06 & 0.34$\pm$ 0.06 & 0.46$\pm$ 0.07 &  
0.54$\pm$ 0.03 & 0.16$\pm$ 0.03 & 0.23$\pm$ 0.02 &  
0.72$\pm$ 0.16 & 0.57$\pm$ 0.16 & 0.62$\pm$ 0.13 & 0.49\\

Qwen-VL&	ViT-bigG/14&	Qwen-7B&	0.88$\pm$ 0.11&	0.56$\pm$ 0.11&	0.68$\pm$ 0.09&	0.40$\pm$ 0.17&	{0.48}$\pm$ 0.17&	{0.42}$\pm$ 0.14&	0.12$\pm$ 0.10&	{0.25}$\pm$ 0.10&	{0.16}$\pm$ 0.06&	0.72$\pm$ 0.16 &	0.67$\pm$ 0.16 &	{0.69}$\pm$ 0.12 &	{0.49} \\
LLaVA-1.6-L&	ViT-L/14&	Vicuna-13B-1.5&	0.85$\pm$ 0.17&	0.58$\pm$ 0.17&	0.65$\pm$ 0.07&	0.61$\pm$ 0.23&	0.40$\pm$ 0.23&	0.37$\pm$ 0.09&	0.26$\pm$ 0.20&	0.18$\pm$ 0.20&	0.11$\pm$ 0.04&	0.49$\pm$ 0.15&	{0.71}$\pm$ 0.15&	0.56$\pm$ 0.04&	0.42 \\
MiniGPT-v2&	ViT-G/14&	LLaMA-2-7B& 0.76$\pm$ 0.11& {0.68}$\pm$ 0.11&	 {0.71}$\pm$ 0.08&	0.45$\pm$ 0.06&	0.16$\pm$ 0.06&	0.23$\pm$ 0.07&	0.21$\pm$ 0.02&	0.03$\pm$ 0.02&	0.05$\pm$ 0.03&	 0.69$\pm$ 0.07 &	0.48$\pm$ 0.07 &	0.57$\pm$ 0.08&	0.39 \\
LLaVA-1.6&	ViT-L/14&	Vicuna-7B-1.5&	0.85$\pm$ 0.18&	0.57$\pm$ 0.18&	0.64$\pm$ 0.08&	0.70$\pm$ 0.10&	0.15$\pm$ 0.10&	0.21$\pm$ 0.09&	0.36$\pm$ 0.03&	0.02$\pm$ 0.03&	0.03$\pm$ 0.03&	 0.68$\pm$ 0.20&	0.63$\pm$ 0.20&	0.61$\pm$ 0.08&	0.37 \\
MPlug-Owl2&	ViT-L/14&	LLaMA-2-7B&	0.93$\pm$ 0.08&	0.34$\pm$ 0.08&	0.50$\pm$ 0.09&	0.70$\pm$ 0.04&	0.08$\pm$ 0.04&	0.14$\pm$ 0.06&	0.33$\pm$ 0.01&	0.01$\pm$ 0.01&	0.01$\pm$ 0.01&	0.88$\pm$ 0.18&	0.51$\pm$ 0.18&	0.63$\pm$ 0.14&	0.32 \\

InstructBLIP&	ViT-G/14&	Vicuna-7B-1.1&	0.89$\pm$ 0.20&	0.42$\pm$ 0.20&	0.54$\pm$ 0.19&	0.71$\pm$ 0.04&	0.06$\pm$ 0.04&	0.09$\pm$ 0.06&	{0.38}$\pm$ 0.01&	0.01$\pm$ 0.01&	0.01$\pm$ 0.01&	 0.74$\pm$ 0.05&	0.48$\pm$ 0.05&	0.58$\pm$ 0.06&	0.31 \\
InstructBLIP-L&	ViT-G/14&	Vicuna-13B-1.1& 0.96$\pm$ 0.14&	0.21$\pm$ 0.14&	0.32$\pm$ 0.19&	0.64$\pm$ 0.05&	0.17$\pm$ 0.05&	0.26$\pm$ 0.07&	0.32$\pm$ 0.01&	0.03$\pm$ 0.01&	0.05$\pm$ 0.02&	0.83$\pm$ 0.14&	0.36$\pm$ 0.14&	0.48$\pm$ 0.13&	0.28 \\
LLaVA-1.5-L&	ViT-L/14&	Vicuna-13B-1.5& 0.96$\pm$ 0.07&	0.27$\pm$ 0.07&	0.42$\pm$ 0.08&	{0.72}$\pm$ 0.02&	0.05$\pm$ 0.02&	0.10$\pm$ 0.04&	0.24$\pm$ 0.01&	0.01$\pm$ 0.01&	0.02$\pm$ 0.02&	{0.93}$\pm$ 0.21&	0.42$\pm$ 0.21&	0.54$\pm$ 0.21&	0.27 \\
LLaVA-1.5&	ViT-L/14&	Vicuna-7B-1.5&	0.95$\pm$ 0.10&	0.30$\pm$ 0.10&	0.44$\pm$ 0.11&	0.71$\pm$ 0.03&	0.04$\pm$ 0.03&	0.08$\pm$ 0.06&	0.30$\pm$ 0.00&	0.01$\pm$ 0.00&	0.01$\pm$ 0.01&	0.90$\pm$ 0.19&	0.41$\pm$ 0.19&	0.53$\pm$ 0.18&	0.27 \\

LLaVA-1.1&	ViT-L/14&	Vicuna-7B-1.1& 	{0.98}$\pm$ 0.05&	0.07$\pm$ 0.05&	0.13$\pm$ 0.09&	0.69$\pm$ 0.00&	0.01$\pm$ 0.00&	0.02$\pm$ 0.01&	0.27$\pm$ 0.01&	0.00$\pm$ 0.01&	0.01$\pm$ 0.01&	 0.84$\pm$ 0.15 &		0.26$\pm$ 0.15&		0.38$\pm$ 0.16 & 0.14\\
        

        
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Mode-oriented performance of varied MLLMs on \phd}.
    %, Models are ranked in descending order by the overall PhD score. 
    The best open-source model per mode is highlighted in green. Values after the symbol $\pm$ indicate the standard deviation across the five tasks.
    %, and the top value in each column is bolded. 
    %Values after the symbol $\pm$ indicate the standard deviation across the five tasks.
    }
    \label{exp-all}
\end{table*}

==> AnonymousSubmission/tables/table-exp-hitem.tex <==

\begin{table}[h]
    \ra{1.1}
    \centering
    \begin{adjustbox}{max width=\linewidth}
    \begin{tabular}{@{}lrrrrrrrrrr@{}}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Object Rec.}} & \multicolumn{2}{c}{\textbf{Attribute Rec.}} & \multicolumn{2}{c}{\textbf{Sentiment Und.}} & \multicolumn{2}{c}{\textbf{Counting}} & \multicolumn{2}{c}{\textbf{Positional Rea.}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(l){10-11}
        & C-h & R-h & C-h & R-h & C-h & R-h & C-h & R-h & C-h & R-h \\
        \midrule
        LLaVA-1.5 & & & & & & & & & & \\
        Qwen-VL & & & & & & & & & & \\
        InstructBLIP & & & & & & & & & & \\
        MiniGPT-v2 & & & & & & & & & & \\
        MPlug-owl2 & & & & & & & & & & \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{\textbf{Performance (PhD score) of MLLMs on Various Tasks and Textual Items}. The tasks include object recognition, attribute recognition, sentiment understanding, counting, and position reasoning. ``C-h'' represents CLIP-based hitems, while ``R-h'' denotes random-based items.}
\end{table}


==> sec/backup-exp.tex <==
\subsection{Results}

\subsubsection{How MLLMs Perform given Visual Ambiguity?}

Results are shown in Table \ref{exp-all}.

\textbf{Results on VHE-base.}
MiniGPT4-v2 achieves the highest F1 score among open-source models at 0.71, though it still trails behind GPT-4o’s 0.84. 

Task-specific performance details for VHE-base are provided in the appendix. Across tasks, MLLM performance declines with task complexity; for example, MiniGPT-4 v2 achieves F1 scores of 0.86, 0.71, 0.69, 0.66, and 0.64 for object, attribute, sentiment, positional recognition, and counting, respectively.

A comparison of model sizes (e.g., LLaVA-1.5, LLaVA-1.6, InstructBLIP) shows that increasing LLM scale doesn’t consistently improve VHE-base performance and may even reduce it. For example, LLaVA-1.5 achieves an F1 score of 0.44, slightly higher than LLaVA-1.5-L’s 0.42, while InstructBLIP scores 0.54 compared to InstructBLIP-L’s 0.32. In contrast, visual component enhancement yields clearer benefits: LLaVA-1.6 (with higher-resolution inputs) and MiniGPT4-v2 and Qwen-VL (both using larger ViT-G models) perform better on VHE-base.  An exception is InstructBLIP, which, despite using ViT-G, scores only 0.54, likely due to overfitting issues \cite{xu2023lvlm}. These results confirm our analysis that VHE-base primarily reflects hallucinations from visual ambiguity, emphasizing the importance of improved visual capability.



\begin{figure*}[h]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/figures/plot_radar_0.pdf}
        \caption{PhD-base}
        \label{fig:radar0}
    \par\bigskip  % 控制行间距
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/figures/plot_radar_1.pdf}
        \caption{PhD-iac}
        \label{fig:radar1}
    \end{subfigure}
    \par\bigskip  % 控制行间距
    % 第三行子图
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/figures/plot_radar_2.pdf}
        \caption{PhD-icc}
        \label{fig:radar0}
    \par\bigskip  % 控制行间距
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AnonymousSubmission/figures/plot_radar_3.pdf}
        \caption{PhD-ccs}
        \label{fig:radar1}
    \end{subfigure}
    \label{fig:comparison_radar}
\end{figure*}


\subsubsection{\phd~ versus Predecessors}

Unlike previous VHE datasets, PhD is designed specifically around the causes of hallucination, making it more challenging. As shown in Table \ref{evolution}, other VHE datasets reach performance saturation quickly as LLaVA models are iteratively updated, achieving results close to GPT-4o. For instance, the performance gap between LLaVA-1.6-L and GPT-4o on POPE and AMBER is only 2.3\% and 8.0\%, respectively. However, on the PhD dataset, the performance gap remains substantial—exceeding 40\%—highlighting the considerable difference between even the latest LLaVA model and GPT-4o, a distinction not observed in other VHE datasets. 

\begin{table}[ht]
\ra{1}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}lrrr@{}}
\toprule
\textbf{Model} & \textbf{POPE} & \textbf{AMBER} & \textbf{PhD}  \\
\midrule
LLAVA-1.1 & 0.67 (-23.9\%) & 0.33 (-62.1\%) & 0.14 (-81.6\%)  \\ 
LLAVA-1.5 & 0.84 (-4.5\%) & 0.75 (-13.8\%) & 0.27 (-64.5\%)  \\ 
LLAVA-1.5-L & 0.85 (-3.4\%) & 0.73 (-16.1\%) & 0.27 (-64.5\%) \\ 
LLAVA-1.6 & 0.87 (-1.1\%) & 0.79 (-9.2\%) & 0.37 (-51.3\%)\\ 
LLAVA-1.6-L & 0.86 (-2.3\%) & 0.80 (-8.0\%) & 0.42 (-44.7\%) \\ 
GPT-4o & 0.88 & 0.87 & 0.76\\ 
\bottomrule
\end{tabular}
}
\caption{\textbf{Performance comparison of MLLMs across three VHE benchmarks.} We select the LLaVA series to illustrate performance differences relative to GPT-4o, with the performance gap shown in parentheses as a percentage. Each dataset uses its recommended metrics.}
\label{evolution}
\end{table}



\textbf{Evaluation modes in \phd~are complementary}. 
The evaluation modes in \phd~target distinct causes of hallucination, making them complementary and collectively forming a comprehensive VHE. As shown in Table \ref{exp-all} and visualized in Figure \ref{fig:comparison_bar}, there are notable performance differences across modes, and the model performance rankings vary significantly. For example, MPlug-Owl2 ranks lower on VHE-base yet leads on VHE-ccs. Performance levels also differ notably: while most models score above 0.4 on VHE-base, many score close to zero on VHE-icc. Interestingly, VHE-iac and VHE-icc exhibit similar trends, as they address the same cause of hallucination but differ in intensity. Thus, these four evaluation modes support each other, providing complementary insights.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{AnonymousSubmission/figures/plot_bar.pdf}
    \caption{\textbf{Performance bar across four evaluation modes.} We present results for MLLMs with LLM sizes of 7B.}
    \label{fig:comparison_bar}
\end{figure}


\subsubsection{How MLLMs Perform given Inaccurate Context?}


\textbf{Results on VHE-iac.}
Compared to VHE-base, all open-source MLLMs show a substantial performance drop, with the top model, Qwen-VL, reaching only an F1 score of 0.42.  Since VHE-iac is directly comparable to VHE-base—differing only by the addition of a slightly inaccurate textual context—this sharp decline suggests that even minimal textual noise can strongly affect model performance, greatly limiting MLLMs’ effectiveness in complex interaction modes such as handling long contexts and multi-turn dialogues.

Although GPT-4o is also affected, its performance declines only slightly (from 0.84 to 0.75). GPT-4o’s substantial advantage over open-source MLLMs in this mode highlights the need for further research into reducing biases introduced by multi-modal inputs in MLLMs.


\subsubsection{How MLLMs Perform given Incorrect Context?}

\textbf{Results on VHE-icc.}
Performance declines even further in this mode compared to VHE-iac, with many MLLMs (\eg, MPlug-Owl2, InstructBLIP, LLaVA-1.1, LLaVA-1.5) scoring close to zero. This trend suggests that as models favor the text modality, they tend to ignore image content when conflicts arise between text and image inputs. Even with an explicit prompt added before each question—``In case of a conflict, prioritize the image content"—the models still fail to shift their attention to the image. Nearly all open-source models struggle in this mode. In contrast, GPT-4o successfully follows the prompt instructions, demonstrating a clear advantage in handling multi-modal input conflicts.

% A comparison between VHE-base, VHE-iac, and VHE-icc reveals a noticeable decline in performance across all MLLMs. The key difference among these three modes lies in the context provided: no context, inaccurate context, and incorrect context, respectively, while the questions asked remain consistent. This variation in performance underscores the significant issue of modality imbalance that contributes to VH.

\subsubsection{How MLLMs Perform given CCS Content?}

%\textbf{Results on VHE-ccs.} 
In the VHE-ccs mode, we observe that improved visual capability can enhance performance to some extent, but the effect is inconsistent. For instance, although MPlug-Owl2 performs poorly on VHE-base due to its weaker visual model, it surpasses MiniGPT4-v2 on VHE-ccs (0.63 vs. 0.57). We conducted additional experiments with the CLIP model to investigate this aspect in greater detail, see Appendix.
Additionally, increasing LLM size proves ineffective for improving VHE-ccs performance; in models like LLaVA-1.5, LLaVA-1.6, and InstructBLIP, larger LLM sizes generally correspond to lower performance.

VHE-ccs reveals a deeper hallucination challenge: conflicts between image content and the model's internal knowledge. Solving this issue requires a comprehensive approach, going beyond isolated improvements to visual or language components. Instead, it calls for a multi-faceted strategy involving data, training processes, and model architecture adjustments.

% The best open-source model, Qwen-VL, performs similarly to GPT-4o, with scores of 0.75 and 0.79, respectively. To explore the source of hallucinations, we used CLIP to calculate image-text similarities between CCS images and both CS and CCS descriptions. Detailed processes are in the appendix. The results show average scores of 0.21 for CS and 0.26 for CCS, suggesting that CLIP captures counter-common-sense content, with hallucinations likely stemming from the LLM's internal knowledge overshadowing visual input.




% Performance differences stem from the feature granularity required. Coarse-grained tasks like object and attribute recognition perform well with existing MLLMs, while finer-grained tasks like counting and position recognition show lower performance.

\textbf{Is larger LLM a bless or a curse?} 
Typically, larger models are associated with better performance. However, this assumption does not necessarily hold on the VHE. As shown in Figure \ref{fig:dis}, we visualize the performance of LLaVA-1.5, LLaVA-1.6, and InstructBLIP across different model sizes (7B and 13B) using box plots. Notably, on VHE-base and VHE-ccs, larger models actually perform worse. This aligns with their design sources, as VHE-base emphasizes visual capability, and VHE-ccs focuses on counter-common-sense images. In these modes, larger models appear to neglect crucial visual content. Conversely, on VHE-iac and VHE-icc, larger models demonstrate improved performance, likely due to their enhanced ability to interpret user instructions, which prioritizes visual content (see the evaluation prompts in Section \ref{exp-cs}).



% According to Table \ref{exp-all} and Figure \ref{fig:Comparison}, increasing LLM size benefits VHE-iac. Larger LLMs exhibit stronger contextual understanding, enabling them to discern that inaccurate context has minimal impact on image comprehension, allowing for better focus on the image itself. However, in VHE-icc mode, these benefits are limited due to the direct conflict between context and image content. Notably, Qwen-VL achieved the highest performance in both VHE-iac and VHE-icc modes despite using only a 7B LLM. As for VHE-base and VHE-ccs modes, increasing model size may potentially harm performance, indicating that these modes rely more on the visual module, and larger LLMs may face greater adaptation challenges. In summary, while increasing LLM size aids in context understanding, addressing visual hallucinations relies more on improving the visual module and optimizing its adaptation with LLMs.


% The findings indicate that simply increasing the size of LLMs does not effectively address the issue of visual hallucinations (see the results from VHE-base and VHE-CCS). This limitation arises because many visual tasks require finer-grained visual features, which cannot be adequately captured by enhancements focused solely on LLMs. Moreover, even though ViT can extract relevant CCS visual information (as indicated by its better alignment with CCS descriptions), these features are often disregarded by LLMs due to internal knowledge conflicts.

% \textbf{}


\textbf{\phd~score is significant}.  
Although \phd~uses a binary question format, \phd~score design ensures minimal impact on evaluation results. For example, LLaVA-1.1 answers ``Yes'' to nearly all questions on VHE-base, resulting in an original F1 score of 0.68, while LLaVA-1.5 scores 0.72, which is very close. In contrast, when using the PhD score as the metric, there is a clear difference between the two models (0.13 vs. 0.44).
Despite the simplicity of binary questions, all open-source models perform poorly on \phd. Notably, more advanced models, like GPT-4o, exhibit a more balanced Yes/No response ratio, which may help mitigate the VH problem.

